MiCS: Near-linear Scaling for Training Gigantic Model on Public Cloud

Existing general purpose frameworks for gigantic model training, i.e., dense models with billions of parameters, cannot scale efficiently on cloud environment with various networking conditions due to large communication overheads. In this paper, we propose MiCS, which Minimizes the Communication Scale to bring down communication overhead. Specifically, by decreasing the number of participants in a communication collective, MiCS can utilize heterogeneous network bandwidth, reduce network traffic over slower links, reduce the latency of communications for maintaining high network bandwidth utilization, and amortize expensive global gradient synchronization overhead. Our evaluation on AWS shows that the system throughput of MiCS is up to 2.89$\times$ that of the state-of-the-art large model training systems. MiCS achieves near-linear scaling efficiency, which is up to 1.27$\times$ that of DeepSpeed. MiCS allows us to train a proprietary model with 100 billion parameters on 512 GPUs with 99.4% weak-scaling efficiency, and it is able to saturate over 54.5% theoretical computation power of each GPU on a public cloud with less GPU memory and more restricted networks than DGX-A100 clusters.

==> Makefile <==
.PHONY: all clean dist print

P = main

default : $P.pdf

$P.dvi	: $(wildcard *.tex *.bib figures/*.eps)
	latex  $P < /dev/null || $(RM) $@
	bibtex $P < /dev/null || $(RM) $@
	latex  $P < /dev/null || $(RM) $@
	latex  $P < /dev/null || $(RM) $@

quick  : $(wildcard *.tex sections/*.tex *.bib figures/*)
	pdflatex --shell-escape $P
	rm -f *.aux *.log *.out *.bbl *.blg *~ *.bak $(FIGS) $(TARGET).ps $(TARGET).synctex.gz
	if which xdg-open 1>/dev/null 2>&1; then \
		xdg-open $P.pdf; \
	else \
		open -a Preview $P.pdf & \
	fi

$P.pdf  : $(wildcard *.tex sections/*.tex *.bib figures/*)
	pdflatex --shell-escape $P
	bibtex $P
	pdflatex --shell-escape $P
	pdflatex --shell-escape $P
	rm -f *.aux *.log *.out *.bbl *.blg *~ *.bak $(FIGS) $(TARGET).ps $(TARGET).synctex.gz
	if which xdg-open 1>/dev/null 2>&1; then \
		xdg-open $P.pdf; \
	else \
		open -a Preview $P.pdf & \
	fi

$P.ps	: $P.dvi
	dvips -tletter -Ppdf $P.dvi -o $P.ps

$P.ps.gz: $P.ps
	$(RM) $P.ps.gz
	gzip -9 < $P.ps > $P.ps.gz

print:	$P.ps

dist:	$P.ps.gz

clean:
	$(RM) $P.log $P.aux $P.bbl $P.blg $P.out $P.dvi $P.ps $P.ps.gz texput.log


==> sections/vldb-response-to-reviewers.tex <==
\section*{Response to Reviewer Comments}

We sincerely thank all the reviewers for their time and comments! We have revised our paper accordingly. The revised parts are marked with color \zhen{blue}. In the remainder of this section, we respond to each reviewer's comments in order. For each comment, hyperlinks to the modified contents are available in the response. 

\subsection*{Towards Reviewer \#1's Comments}
\parabf{Comments \#1}: \emph{ Limited in-depth comparison to prior DNN training and, even more so, general distributed compute approaches:
- The empirical comparison is primarily anchored on one prior approach, ZeRO, and the overall discussion of tradeoffs relative to this approach as well as others seems fairly minimal;
- A more thorough comparison to how the proposed approaches relate to the broader field of literature on distributed compute (not necessarily large DNN model training related) would have been appropriate. } 

\parabf{Responses \#1}: 
For the concern about comparing to broader literature in distributed computing,
we revised the paper to include more discussions with respect to the communication optimization techniques used in the high-performance computing community, which we believe is one of the most relevant subfields to us in distributed computing. Specifically, we discussed the several advancements in hardware and optimizations that choose different algorithms for different sized messages. The discussion of the relations to our work is included in the last part of the related work \S\ref{sec:related-comm-optim}. % \yida{this is too brief, compared to the previous paragraph. (Zhen: Extended)}

Regarding the concern of the empirical evaluations, we agree it would be beneficial to broadly compare to prior DNN training systems. While most of the prior data-parallel training systems~\cite{sergeev2018horovod,byteps,bytescheduler_impl} are not able to take the workloads that we are targeting (\S\ref{sec:large_model_training}). The DeepSpeed/ZeRO system is picked for its ability to support training for large models with pure data parallelism strategies, which is the focus of \sysname. More discussions are available at the \S\ref{sec:large_model_training} and \S\ref{sec:introduction}. For completeness, we have also compared to state-of-the-art systems with other parallelisms included at \S\ref{sec:eval_compare_megatron} and \S\ref{sec:eval:wide-resnet}. Towards the trade-offs to other parallelism strategies, we revised the paper with additional experiments and discuss it in the next response.

% \sysname is a pure data-parallel training solution. Thus, the evaluation mainly compares \sysname with respect to other data-parallel systems. Most prior data-parallel training systems are designed for relatively smaller models, which can be fit into a single GPU for training. But the targeted models of our system have billions of parameters that cannot fit into a single GPU for training. For example, the 10B BERT model requires at least 160GB GPU memory for training with half-precision and Adam optimizer. The relevant discussion is in the first part of the introduction and the ``Data parallelism'' section of related work. DeepSpeed is a well-engineered data-parallel training system that can support large model training by ZeRO partition strategy (We revised \S\ref{sec:large_model_training} with more details). Thus, it is the most relevant solution for us to compare with. For completeness, we have also compared with Megatron-LM-3D, which combines model, data, and pipeline parallelisms, and is considered as the state-of-the-art implementation for transformers-based models. We discussed differences and trade-offs between model-parallel systems and data-parallel systems in \S\ref{sec:large_model_training}. The evaluation results in \S\ref{sec:eval_compare_megatron} and \S\ref{sec:eval:wide-resnet} show that the \sysname achieves good performance and is more general than the model-parallel based solution. \yida{all above seems well-taken by the reviewers. No doubt about what we have done.}




\parabf{Comments \#2}: \emph{Limited exploration of intentional design tradeoffs: 
- As the authors mention in Section 7, there are design tradeoffs between this and prior approaches, some claimed by the authors to have been intentional;
- These tradeoffs should have ideally gotten more attention in the experiments (not just ablations of component-wise contributions)}

\parabf{Response \#2}: In response to the suggestions, we first add additional experiments in \S\ref{sec:eval_compare_megatron}, to justify the claim that there is a limitation of \sysname with respect to other systems with model parallelism. The descriptions for the additional experiments are presented in the last part of \S\ref{sec:eval_compare_megatron}. And we expanded the corresponding discussion in the first part of \S\ref{sec:limit}.

%For comparing our system with prior ZeRO systems, we used the inaccurate statement that ``\sysname trades the memory consumption for lower the communication costs'' in the last version. The more accurate statement would be ``\sysname utilizes spare memory resource for lower the communication costs''. This isn't an intentional ``trade-off''. We apologize for the confusion. The revised statement has been made in the second paragraph of \S\ref{sec:limit}.
The reviewer's comment also helps us realize that our statement ``\sysname trades the memory consumption for lower the communication costs'' is less accurate.
It is indeed not a ``trade-off'' but an improvement.
We hence revise the statement to be ``\sysname utilizes spare memory resource for lower the communication costs''.
The revised statement has been made in the second paragraph of \S\ref{sec:limit} to remove the ambiguity from the previous version.

% \todo{Expand the Section 7 to include more detailed explantion about trade-off to ZeRO-3, which is not exactly the trade-off. For the trade-off towards MP solution, DP solution require each GPU at least process one sample, thus if intermediate activations are large could result in OOM issue, TP could mitigate this problem due to the partitioned activation. }

\parabf{Comments \#3}: \emph{Heuristic hyperparameters: several hyper-parameters are heuristically chosen; though this is acknowledged and left for future work, this seems like a significant omission for a complete system in practice?}

\parabf{Response \#3}: 
We agree that including an automated procedure for hyperparameter tuning would further alleviate the burden on the user side. However, the challenges presented in automating configuration search are orthogonal to the focus of the paper. Estimating runtime memory consumption, as an essential component for configuration search, is challenging due to the dynamic graph dispatching and memory management of the underlying runtime system. In this paper, we focus on the communication bottleneck of the ZeRO DP method in large-scale clusters. To make it clear, we revised the corresponding content in the last two paragraphs in \S\ref{sec:limit}.

% \zhen{Nowadays, it is common that users choose hyperparameters heuristically when using large model training systems in practice. For example, to do training with Megatron-LM-3D, users need to figure out the size of tensor MP size and pipeline MP size to fit the model in each device, based on manual estimation and inspection. ZeRO system follows similar practice. We revised the paper to include the discussion in the third paragraph of \S\ref{sec:limit}. }
% \yida{this paragraph is not quite needed. We don't need to argue with the reviewer, just acknowledge his/her point and revise the paper. If we want to argue that this is NOT a significant omission, we should soften the tone. (Zhen: modified)}



% \begin{itemize}
%     \item The completeness of \sysname doesn't fall behind prior systems, DeepSpeed or Megatron-LM-3D. For a given training setup, users have to figure out the size of the cluster for training first. 
%     \item The heuristic rule follows the core principle of \sysname.
%     \item To automating the configuration search process, we need to have accurate estimation for the memory requirement, which is hard for systems built on top of runtime system using dynamic graphs like PyTorch. The challenges include inaccurate memory estimation, time-consuming for profiling based method, and difficult to clean up the environment if the job fails. Those challenges are orthogonal to communication bottleneck when scaling out the cluster.
% \end{itemize}


\subsection*{Towards Reviewer \#2's Comments}
\parabf{Comments \#1}: \emph{Substantive experiments and revisions to the claims in the paper regarding limited bandwidth on cloud instances. The claims that cloud providers do not have high bandwidth interconnects does not appear to be grounded in fact. This must be dealt with thoroughly. }

\parabf{Response \#1}: 
We totally agree that cloud providers could have high bandwidths interconnects. The previous version might cause misleading impression that ``public cloud = low bandwidth'' in the first place. We have made corresponding changes. Specifically, when motivating our work in \S\ref{sec:introduction} and \S\ref{sec:comm_overheads}, we put more concrete qualification words to specify cloud networks that we are working with.
It is not our intent to claim that high bandwidth interconnects are not available to the cloud. Instead, our intention is to state the fact that the design of ZeRO systems is not suitable for clusters with less preferable network conditions. 
It is common to see that less ideal network conditions for ZeRO system to run on the cloud-based GPU clusters.
Table~\ref{tab:cloud-vm-types-v100} and Table~\ref{tab:cloud-vm-types-a100} in this rebuttal letter give the number of instance types that provide network bandwidth larger than that reported in our paper (The order of the cloud provider is based on the recent report of market share in cloud computing~\cite{cloud-share-report-2022}). Roughly speaking, there is no cloud instance equipped with V100 GPUs that can provide network bandwidth larger than 100Gbps. In comparison, the ZeRO systems~\cite{ms_zero} are evaluated on DGX-2 nodes with 800Gbps InfiniBand network for V100 GPUs. Besides, many cloud networks have relatively higher peer-to-peer latency as compared to InfiniBand~\cite{ziegler2022efa-dbms-latency}, which negatively impact the network utilization on real workloads. These facts cause large communication overhead when adopting ZeRO systems in cloud-based GPU cluster with 100Gbps or 400Gbps networks. This motivates us to redesign the ZeRO system to reduce the communication overhead and preserve the simplicity and generality of partitioned DP methods. Our evaluation results show that \sysname achieves state-of-the-art performance numbers in less ideal network environments, i.e., A100(40GB) GPUs with 400Gbps networks, in comparison with A100(80GB) GPUs with 1.6Tbps networks. We believe that \sysname provides a positive impact for large model training in the cloud network environment in general.

% We agree with the comments that our paper should carefully present the fact of the network environment on the public cloud. We thus revised our paper accordingly.  %\todo{Need to see which part need to revise. potentially remove the ``public cloud'' in title?}.

Regarding the network bandwidth on cloud TPUs, we'd like to kindly point out that, the ``bisection bandwidth per Pod'', provided by the TPUv4 specifications, is not the same as per virtual machine network bandwidth. The bisection bandwidth per Pod is calculated for TPU chips interconnected within a Pod. It is not the network bandwidth across two Pods. Google didn't release the bandwidth across TPU pods. Thus, we don't know how much faster it would be as compared to GPU instances. Based on the interconnect topology and the bisection of TPUv4, the derived inter-chip interconnect bandwidth is about 47GB/s, which is calculated based on ``bisection-bandwidth / cross-section-links-of-3d-torus = 24000 / (16 * 16 * 2)''.


\begin{table}
    \centering
    \small
    \caption{The number of instance types with V100 GPUs and network bandwidth higher than 100Gbps; ``BW'': bandwidth. }
    \label{tab:cloud-vm-types-v100}
    \begin{tabular}{l r r r}
    \toprule
    Cloud provider & \# types w/ BW $>$ 100Gbps  & total \# of types \\
    \midrule
    Amazon & 0  & 4 \\
    Azure & 0  & 5 \\
    Google Cloud & 0 & 4 \\
    \bottomrule
    \end{tabular}
\end{table}

\begin{table}
    \centering
    \small
    \caption{The number of instance types with A100 GPUs and network bandwidth higher than 400Gbps; ``BW'': bandwidth. }
    \label{tab:cloud-vm-types-a100}
    \begin{tabular}{l r r r}
    \toprule
    Cloud provider & \# types w/ BW $>$ 400Gbps  & total \# of types \\
    \midrule
    Amazon & 0  & 2 \\
    Azure & 2  & 5 \\
    Google Cloud & 0 & 5 \\
    \bottomrule
    \end{tabular}
\end{table}

% \begin{itemize}
%     \item Acknowledge for bringing the attention of high bandwidth availability on public cloud
%     \item The bisection bandwidth of TPU pods are not directly comparable to network bandwidth of cloud VM instances. For one pod contains 4096 TPU chips, the available bandwidth for TPUv3 is about XX. TPUv4 is still in the preview. 
%     \item Azure's A100 instances are not generally available to the public, but require an on-premise contract. \todo{Need to verify, but based on the Azure console, high bandwidth instances are not available. }
%     \item List of currently available GPU instances with network bandwidth specifications.
%     \item In general, we want to convey the idea that with less ideal network bandwidths, we can scale efficiently well. 
% \end{itemize}

\parabf{Comments \#2}: \emph{Substantive experiments or revisions to the claims that the paper deals with ``gigantic models''. The authors should benchmark other kinds of tasks, e.g., the MLPerf tasks, or revise the claims in the paper.}

\parabf{Response \#2}: 
We apologize that we didn't make it clear about the types of models we target.
We made the modification in \S\ref{sec:large_model_training} to include a more precise definition of what we refer to as ``gigantic models''. Basically, a gigantic model is large in two aspects: 1) the size of the model states cannot fit into a single GPU for training, which typically means that the model has at least one billion parameters when training with the Adam optimizer; 2) the majority of the parameters of the model are connected densely, which means the operational intensity~\cite{williams2009roofline}, i.e., operation/bytes, of the model is large.

When we looked into the MLPerf benchmarking models, we found that most of the models can fit into a single V100 (32GB) GPU in training.
Models in MLPerf mostly consist of far less than one billion parameters. DLRM, as an exception, has billions of parameters. However, only a very small fraction ($~0.01\%$) of model parameters are in dense layers. The majority of the parameters are in Embedding layers and activated sparely in the training procedure. This results in low FLOPs of each sample in training (about 1.42e+7 FLOPs/sample), or in other words, the operational intensity is near-zero (9.85e-5 FLOPs/byte), which requires a different set of optimization techniques.
In comparison, the BERT 10B model (in Table~\ref{tab:eval_model_structures}) in our evaluation has 4.1e+13 FLOPs/sample, corresponding to per sample operational intensity of the model is about 2048 FLOPs/byte.

We summarize the number of parameters of MLPerf tasks as follows for reference purposes.
\begin{itemize}
    \item ResNet-50 (v1.5): 25.6 million parameters.
    \item 3D U-Net: 31.1 million parameters.
    \item SSD: 37.0 million parameters.
    \item Mask R-CNN: 44.44 million parameters.
    \item RNN-T: 49 million parameters.
    \item BERT-large: 336 million parameters.
    \item DLRM(1TB data): 24 billion parameters in total, 2.4 million parameters in dense layers.
\end{itemize}


% \begin{itemize}
%     \item We consider "gigantic" in terms of memory and computations. The model states cannot fit into a single GPU or a single computational node, and has a large number of float operations in training, i.e., dense computation. 
%     \item Give table for presenting size and FLOPs of models in the MLPerf tasks. 
% \end{itemize}
% We apologize for the vague definition of "gigantic models". Specifically, we are considering dense models with billions of parameters that cannot fit into a single GPU or a single computational node for training. The target workloads of our system are beyond the scope of MLPerf. The largest model size of MLPerf tasks is XX, which has YY parameters and is trainable on single V100 (32GB) GPU. Recently, transformer-based models are the most common way to scale up the model sizes~\cite{XX}. And this model structure has been successfully applied in various fields including computer vision, speech recognition, natural language processing. Thus, we believe the workloads we used are representative and valuable~\cite{X}. To demonstrate the generality of the system, we included experiments for WideResNet~\ref{X}, which is another way of scaling up the model size. And in Section~\ref{X}, \sysname achieves good scalability efficiency as well. 


\parabf{Comments \#3}: \emph{Time-to-accuracy experiments. The authors make claims that prior work affects convergence, which is in direct opposition to the claims of the previous work. Such claims must be substantiated with experiments. Similarly, the authors should perform time-to-accuracy experiments on their algorithm, if they plan to keep such claims.}

\parabf{Response \#3}:
For the concern about the correctness of the claim in our paper that ``asynchronous and bounded-staleness training affect convergence'', 
we agree that including supporting evidence would be better in the context. We thus revised the related work to include theoretical studies of asynchronous algorithms. The paper suggested in the comments also provides evidence
that the asynchronous methods change the semantic of the training procedure~\cite{analysis-DAWNBench}, which affects the time-to-accuracy (TTA) convergence. Thus, TTA check is important to asynchronous training methods. The convergence of asynchronous methods may vary significantly on different datasets, refer to Table 2 of PipeMare~\cite{pipemare_mlsys21}. Theoretical studies of optimization algorithms~\cite{recht2011hogwild, de2015taming} also show the convergence gap between asynchronous training and synchronous training. Due to the aforementioned side effects of asynchronous training, systems widely adopted by the industry use synchronous training~\cite{tensorflow,sergeev2018horovod,byteps,rasley2020deepspeed,megatron_lm,megatron_lm_3d}. Besides, our work focuses on communication bottleneck in partitioned data parallel methods, which is orthogonal to the research of asynchronous training algorithms. We can potentially incorporate asynchronous methods into \sysname.

Towards the evaluation metrics, we believe throughput performance, TFLOPS saturation, and scaling efficiency (including weak scaling and strong scaling) are commonly used metrics in the literature~\cite{megatron_lm_3d,megatron_lm, ds-megatron-530b,sergeev2018horovod,byteps,alpa,ms_zero,ren2021zerooffload,rajbhandari2021zeroinfinity}. Moreover, \sysname is a fully synchronized training system. Our optimizations do not change the semantics of the training procedure. When evaluating our system and other baselines, we fixed all other training factors. Thus, in our setup, comparing throughput performance is the same as comparing TTA. And in Section-\ref{sec:fidelity_check}, we checked the convergence with respect to DeepSpeed to ensure the correctness of the implementation.

% As pointed out by the reference paper~\cite{analysis-DAWNBench}, which is about the behaviors of different training setups, system optimizations that modify the semantics of the training procedure can impact the final model's accuracy. Thus, the time-to-accuracy (TTA) is used to compare trade-offs of optimizations that \emph{modify the semantic} of the training procedure. The asynchronous distributed training is one of those optimizations that changes training semantics. Lossy gradient compression, e.g., gradient compressions, is another category of such optimizations that change the semantics of training. Other than asynchronous and lossy compression, changing the batch size, learning rate or other hyperparameters of the training algorithm also changes the semantic of the training procedure. For a given set of hyperparameters, training systems that do not change the semantic of the training procedure are supposed to provide the same convergence, unless the implementation is buggy. For example, TensorFlow and PyTorch are supposed to provide the same convergence for a fixed training setup, which includes model structure, optimizer, hyperparameters, dataset, etc. 





As for the comments that ``Different systems can cause differences in convergence'', in our opinion, it is not completely true. The referenced paper~\cite{analysis-DAWNBench} factors training setups into the definition of the ``distributed systems'', e.g., batch size used in training, whether turning on or off the half-precision training. In this case, we agree that the different ``distributed systems'' can result in different convergence. However, typically, the definition of ``distributed systems'' does not contain training setups. In this case, if two ``systems'' do not change the semantic of training for a fixed setup, then two ``systems'' are expected to provide the same convergence. Or if two ``systems'' change the semantic of training in a same way, e.g., using the same lossy compression algorithm, then they should provide the same convergence as well. In our evaluation, all systems use the same setup for training algorithms.



% In our setup, the throughput performance is equivalent to time-to-accuracy metrics. As the reference paper suggested~\cite{X} by the reviewer pointed out, changing the semantic of the training procedure would affect the convergence and the model quality. Our system uses fully synchronized training paradigm and does not use optimizations that reduce precision. Thus, it does not change the semantic of the training algorithm. In comparison, other works using asynchronous gradient synchronization with bounded-staleness or lossy compression algorithms do change the semantic of the training algorithm~\cite{X}. Thus, "time-to-accuracy" is required for those types of works for tracking the convergence. 
% There are some works~\cite{X} discuss the asynchronous and convergence rate. Specifically, with staleness XX the convergence rate will be affected by up to YY~\cite{X}. Because of this kind of uncertainty from the asynchronous system, in the industry use cases, the widely adopted large model training uses synchronous paradigm like DeepSpeed and Megatron-LM-3D. We have also provided sentinel check for the system in the Section~\ref{X}.

\subsection*{Towards Reviewer \#3's Comments}
\parabf{Comments \#1}: \emph{D1. The paper gives a very brief explanation of the communication that happens when training models with model state partitioning (Section 3.2). To understand why communication is excessive when the model state is partitioned across all devices and understand the bottlenecks, the authors need to better explain the communication phases (e.g., parameter gathering, gradient synchronization) and when they are happening (e.g., f/b propagation, parameter update); perhaps a figure or diagram would help.}

\parabf{Response \#1}: 
Following the suggestions from the comments,
we added Figure~\ref{fig:partitioned-dp-zero3} and updated descriptions to explain the ZeRO-3 DP training in \S\ref{sec:large_model_training}. The contents are marked with color blue. 

\parabf{Comments \#2}: \emph{D2. The experimental analysis compares the performance of MiCS and Zero but neglects the fact that MiCS has larger memory requirements; in general, more GPUs are needed to train a model using MiCS than using Zero. How does that reflect in the monetary cost? Does it pay off to acquire more HW resources to be able to use MiCS? The experimental analysis does not consider this aspect, which is very important in the public cloud setting.}

\parabf{Response \#2}: From the comments, we realized that we didn't make it clear that \sysname doesn't require additional hardware resources for training. % the confusing relationship between model states replication and overall resource requirements.
%\yida{this sentence is not clear to me.} 
We revised the discussion of trade-offs with respect to ZeRO systems in the second paragraph of \S\ref{sec:limit}. In short,
ZeRO system underutilizes memory resources. \sysname trades spare memory resources in prior work to lower the overhead of communications. The detailed discussion is available at the first paragraph in \S\ref{sec:sys_design_topo_aware}.

\parabf{Comments \#3}: \emph{D3. Minor comments: 1) typo: Next, We introduce; 2) typo: In addition, We have} 

\parabf{Response \#3}: 
Typos are fixed. 

\clearpage
